Ecological Semantics: Programming Environments for Situated Language Understanding

Large-scale natural language understanding (NLU) systems have made impressive progress: they can be applied flexibly across a variety of tasks, and employ minimal structural assumptions. However, extensive empirical research has shown this to be a double-edged sword, coming at the cost of shallow understanding: inferior generalization, grounding and explainability. Grounded language learning approaches offer the promise of deeper understanding by situating learning in richer, more structured training environments, but are limited in scale to relatively narrow, predefined domains. How might we enjoy the best of both worlds: grounded, general NLU? Following extensive contemporary cognitive science, we propose treating environments as "first-class citizens" in semantic representations, worthy of research and development in their own right. Importantly, models should also be partners in the creation and configuration of environments, rather than just actors within them, as in existing approaches. To do so, we argue that models must begin to understand and program in the language of affordances (which define possible actions in a given situation) both for online, situated discourse comprehension, as well as large-scale, offline common-sense knowledge mining. To this end we propose an environment-oriented ecological semantics, outlining theoretical and practical approaches towards implementation. We further provide actual demonstrations building upon interactive fiction programming languages.

==> conclusions.tex <==
Contemporary cognitive science research illuminates the formative role of rich, interactive environments in shaping cognition and language, and suggests that they must also be integral to computational accounts.  In this position paper, we proposed theoretical and practical approaches to incorporate such insights into current NLU systems. We hope our paradigm could be useful for providing coherence to efforts towards human-like language understanding.



==> formal.tex <==
Mental simulations and affordances feature centrally in contemporary cognitive linguistics research. According to one such theory, the Indexical Hypothesis~\citep{Glenberg2008}, language comprehension involves three key processes: indexing objects, deriving their affordances, and meshing them together into a coherent (action-based) simulation as directed by grammatical cues. Importantly, affordances generally cannot be derived directly from words, but rather rely on context and pre-existing object representations. 

For a more formal computational account, we adopt the model-based framework used in general AI mental simulation research~\citep{Hamrick2019}. At the core of such frameworks is the partially observable Markov Decision Process (POMDP)~\citep{kaelbling1998planning}:\ronen{finish formal notations}

Grounded language learning settings can also be formulated (and often are) within such a framework, where the executor functions as $T$ and the parser maps an input $o\in O$ to program $\left\{ a_{t}\right\} _{t=1}^{T}$.

Importantly, most grounded/executable approaches assume a fixed, domain-specific $T$ (navigation environments, SQL engine, etc.) and focus on learning the policy. 

Our setting, which we term ecological semantic parsing, focuses on the complementary problem of learning $T$:

Ecological Semantic Parsing (EcSP): Given a textual input describing the behavior of an environment, return code implementing the behavior

We argue that a no less important challenge is extending $T$ to be applicable in more general language understanding; indeed, learning $T$ at large-scale is closely related to the grand AI challenge of common-sense learning. In humans, common-sense is hard-coded through rich experience; it is reasonable to expect that large parts of $T$ will require hard-coding as well. How to do so efficiently and at scale? Natural language offers a clue of how such knowledge is represented efficiently by humans: when made explicit, it is through the language of affordances. Indeed, $T$ can be thought of as an affordance function.

Coding $T$ at scale by humans or AIs requires a programming language analog. A promising candidate is the behavioral programming paradigm, which we discuss in the next section.










